A Kernel-Based Explicit Unconditionally Stable Scheme for Hamilton-Jacobi Equations on Nonuniform Meshes

In \cite{christlieb2019kernel}, the authors developed a class of high-order numerical schemes for the Hamilton-Jacobi (H-J) equations, which are unconditionally stable, yet take the form of an explicit scheme. This paper extends such schemes, so that they are more effective at capturing sharp gradients, especially on nonuniform meshes. In particular, we modify the weighted essentially non-oscillatory (WENO) methodology in the previously developed schemes by incorporating an exponential basis and adapting the previously developed nonlinear filters used to control oscillations. The main advantages of the proposed schemes are their effectiveness and simplicity, since they can be easily implemented on higher-dimensional nonuniform meshes. We perform numerical experiments on a collection of examples, including H-J equations with linear, nonlinear, convex and non-convex Hamiltonians. To demonstrate the flexibility of the proposed schemes, we also include test problems defined on non-trivial geometry.

==> space.tex <==
\subsection{Algorithm}

We summarize the proposed scheme in the following algorithm flowchart.

\def\HRule{\rule{\linewidth}{0.1mm}}
\medskip\noindent

{\sf
	\hskip -0.18truein\HRule
	
	\noindent
	\textbf{Algorithm}: Kernel based scheme on nonuniform grids
	\vskip -0.1truein
	\hskip -0.18truein\HRule
	
	\medskip\noindent
	Solve \eqref{c-laws} until the final time $t=T$. Let $N$ be the space mesh size. Denote the mesh, the physical solution, and the transformation Jacobian at $n$-th time step $t=t^n$ %and gridpoint $x=x_{j}$ 
	by 
	$$x^n=\{x^n_{j}\},\text{ }u^n=\{u^n_{j}\}, \text{ and } J^n=\{J^n_{j}\}, \quad j=0,\ldots,N,$$
	respectively. 
	Start with $n=0$ and $t^0=0$.
	
	\noindent
	\begin{enumerate}[label=\textbf{\arabic*.}]
		\setcounter{enumi}{0}
		\item %[{\bf 2.}]
		Given an initial solution at a uniformly distributed mesh, define a monitor function \eqref{Mo2}
		$$M=M_{{u}^{\rm initial}}(x)$$
		with a direct smoothing \eqref{B3} and	 set an adaptive mesh $x^0$ %$\{x^0_{j}\}$
		by de Boor's algorithm.
		Then approximate the associated Jacobian $J^0=x_{\xi}|^{0}$ %$J^0_{j}=x_{\xi}|^{0}_{j}$
		by a sixth-order finite difference scheme,
		and compute the initial solution $u^0$ on initial adaptive mesh $x^0$. %$\{u^0_j\}$ at $\{x^0_j\}$
		
		\item %[{\bf 3.}]
		Set the temporal time step size $\Delta \tilde{t}^0$ by CFL condition \eqref{cfl}.
		
		\item %[{\bf 1.}]
		\cite{HKYY} Find the ideal (linear) weights $d_k$ for the WENO-NE scheme using the equation \eqref{DK} with \eqref{coef1} and \eqref{coef2} : the approximation space %\eqref{bigsp}
		$$\{ 1, \xi,\cos(\lambda \xi),\sin(\lambda \xi),e^{\lambda \xi},e^{-\lambda \xi}\}$$
		is used on a big stencil, and the approximation subspace
		$$\{ 1,\xi,\cos(\lambda \xi),\sin(\lambda \xi)\}$$
		is used on each substencil. The parameter $\lambda>0$ is tunable depending on problems but here it is chosen as $\lambda \Delta \xi=1$ for all experiments.
		
	\end{enumerate}
	
	\medskip\noindent
	While $t<T$, given $x^n$, $u^n$, $J^n$ and $\Delta \tilde{t}^n$  at $t=t^n$,
	\begin{enumerate} [label=\textbf{\arabic*.}]
		\setcounter{enumi}{3}
		\item \label{item4loop} %[{\bf 4.}]
		With an initial guess $\tilde{u}^{n+1}$ by the WENO-NE scheme on mesh $x^{n}$, construct a monitor function \eqref{Mo2} $$M=M_{\tilde{u}^{n+1}}(x)$$
		using a smoothing technique \eqref{B3} several times depending on the problem.
		Then generate a new mesh $\tilde x^{n+1}$ by de Boor's algorithm.
		
		\item % [{\bf 5.}]
		\cite{HRbook, YHQ} Restrict the mesh movement so that the mesh points cannot move too far away from their current locations during one step evolution. In particular, we define a mesh speed as
		\begin{align}\label{xspeed}
		\dot{x}^n_{j}=\frac{\tilde{x}^{n+1}_{j}-x^n_{j}}{\Delta \tilde{t}^n}, \qquad j=1,\ldots,N-1,
		\end{align}
		then the new time step  $\Delta t^n$ is chosen to be
		\begin{align}\label{deltat}
		\Delta t^n \leq  \begin{cases}\displaystyle
		-\frac{1}{2\dot{x}^n_{j}}\left(x^n_{j}-x^n_{j-1} \right), & \text{if $ \dot{x}^n_{j} <0 $}, \\
		\displaystyle
		\frac{1}{2\dot{x}^n_{j}}\left(x^n_{j+1}-x^n_{j} \right),  & \text{otherwise},
		\end{cases}
		\end{align}
		such  that the new mesh $x_{j}^{n+1}$ is restricted inside interval [$x_{j-1/2}^n$, $x_{j+1/2}^n$], i.e.,
		\begin{align*}
		x_{j-1/2}^n =\frac{1}{2}\left( x_{j-1}^{n}+x_{j}^{n} \right) \leq x_{j}^{n+1}=x_{j}^{n}+\Delta t^n \dot{x}_{j}^{n} \leq x_{j+1/2}^n=\frac{1}{2}\left( x_{j}^{n}+x_{j+1}^{n} \right).
		\end{align*}
		
		
		With \eqref{xspeed} and \eqref{deltat}, the mesh $x^{n+1}$ is updated as
		\begin{align*}
		x_{j}^{n+1}=x_{j}^{n}+\Delta t^n \dot{x}_{j}^{n},\qquad j=1,\ldots,N-1.
		\end{align*}
		
		\iffalse	
		\item %[{\bf 6.}]	
		Solve $J^{n+1}$ from the GCL \eqref{gcl} from $t^n$ to $t^{n+1}=t^n+\Delta t^n$ by the WENO-NE scheme described in Section \ref{S-wenone}.
		\item %[{\bf 7.}]
		Solve the transformed hyperbolic conservation law \eqref{hat-claw} from $t^n$ to $t^{n+1}$ for $\hat{u}$ using the same WENO-NE scheme as in the previous step. Here the equation in time is solved using a third-order Runge-Kutta method.
		Finally $u^{n+1}$ is obtained from the relation $u=J^{-1}\hat{u}$.
		\fi
		
		\item %[{\bf 6.}]	
		Solve $J^{n+1}$ and $\hat{u}^{n+1}$ from the GCL \eqref{gcl} and the transformed hyperbolic conservation law \eqref{hat-claw}, respectively, from $t^n$ to $t^{n+1}=t^n+\Delta t^n$ by WENO-NE scheme described in Section \ref{S-wenone}. Finally $u^{n+1}$ is obtained from the relation $u=J^{-1}\hat{u}$; $$u^{n+1}=(J^{n+1})^{-1} \hat{u}^{n+1}.$$
		
		\item %[{\bf 8.}]
		If $t^{n+1}<T$, set
		\begin{align*}
		\Delta \tilde{t}^{n+1}={\rm CFL} \frac{\Delta \xi}{\sup |\hat{f}'(\hat{u})|},
		\end{align*}
		and here, if $t^{n+1}+\Delta \tilde{t}^{n+1}>T$, set $\Delta \tilde{t}^{n+1}=T-t^{n+1}$. With $t=t^{n+1}(=t^n+\Delta \tilde{t}^{n+1})$, go to step \ref{item4loop} and execute the process.
		
		Otherwise, we finish this algorithm.
	\end{enumerate}
	
	\hskip -0.18truein\HRule
}
Here we

\subsection{Space discretization with exponential based WENO schemes}
In this subsection, we present the details about the spatial discretization of $\mathcal{D}_{L}$ and $\mathcal{D}_{R}$.
We denote $L^{*}[v,\gamma](x_{i})$ as $L^{*}_{i}$ on each grid point $x_{i}$, where $*$ can be $L$ and $R$. Note that 
\begin{subequations}
	\label{eq:recursive}
	\begin{align}
	& I^L_i = e^{-\gamma\Delta x_{i}} I^L_{i-1} + J^L_i,\quad i=1,\ldots,N, \quad I^L_0 = 0, \\
	& I^R_i = e^{-\gamma\Delta x_{i+1}} I^R_{i+1} + J^R_i,\quad i=0,\ldots,N-1, \quad I^R_N = 0,
	\end{align}
\end{subequations}
where,
\begin{align}
\label{eq:JLR}
J^L_{i} =  \gamma \int_{x_{i-1}}^{x_{i}} v(y)e^{-\gamma (x_{i}-y)}dy,\ \ \ \
J^R_{i} =  \gamma \int_{x_{i}}^{x_{i+1}} v(y)e^{-\gamma (y-x_{i})}dy.
\end{align}
Therefore, once  $J^{L}_{i}$ and $J^{R}_{i}$ are computed for all $i$, we then can obtain $I^{L}_{i}$ and $I^{R}_{i}$ via the recursive relation \eqref{eq:recursive}.

In \cite{christlieb2017kernel}, we proposed a high order and robust methodology to compute $J^L_{i}$ and $J^R_{i}$. In what follows we briefly review the underlying procedure for completeness of the paper. 

Note that, to approximate $J^L_{i}$ with $k^{th}$ order accuracy, we may choose the interpolation stencil 
$S(i)=\left\{x_{i-r},\ldots,x_{i-r+k} \right\}$,
which contains $x_{i-1}$ and $x_{i}$. There is a unique polynomial $p(x)$ of degree at most $k$ that interpolates $v(x)$ at the nodes in $S(i)$. Then $J^L_{i}$ is approximated by
\begin{align}
\label{eq:linear_JL}
J^L_{i}\approx\gamma \int_{x_{i-1}}^{x_{i}} p(y)e^{-\gamma (x_{i}-y)}dy.
\end{align}
Note that, the integral on the right hand side can be evaluated exactly.
%{\color{red} Usually, we choose the stencil symmetric about $\left\{x_{i-1},x_{i}\right\}$ or one point biased stencil to ensure stability.
%In particular, when the cell $[x_{i-1},x_{i}]$ near the boundary, we can choose the stencil embedded in the domain. Thus this scheme can avoid finding the values on ghost points when treating complicated geometry.}
Similarly, we can approximate $J^R_{i}$ by
\begin{align}
\label{eq:linear_JR}
J^R_{i}\approx\gamma \int_{x_{i}}^{x_{i+1}} p(y)e^{-\gamma (y-x_{i})}dy,
\end{align}
with polynomial $p(x)$ interpolating $v(x)$ on stencil $S(i)=\left\{x_{i+r-k},\ldots,x_{i+r} \right\}$ which includes $x_{i}$ and $x_{i+1}$.

However, in some cases, the linear quadrature formula \eqref{eq:linear_JL} and \eqref{eq:linear_JR} with a fixed stencil may generate the entropy-violating solutions, which will be demonstrated in Section \ref{sec:result}. The main reason is that the viscosity solution of the H-J equation may involve discontinuous derivative. Hence,  an approximation with a fixed stencil such as \eqref{eq:linear_JL} and \eqref{eq:linear_JR} will develop spurious oscillations and eventually lead to failure of the scheme. We found that the WENO quadrature and the nonlinear filter, discussed in \cite{christlieb2017kernel}, are effective to control oscillations and capture the correct solution for solving nonlinear degenerate parabolic equations. In this work, we adapt this methodology to solve H-J equations as both types of equations may develop discontinuous derivatives for the solutions. The numerical evidence provided in Section \ref{sec:result} justifies the effectiveness of the WENO method and nonlinear filter in controlling oscillation as well as in capturing the viscosity solution to the H-J equation. 


In summary, when $\phi_{x}$ is periodic for example, we will use the following modified formulation instead of \eqref{eq:partialsum_per} to approximate $\phi_{x}^{\pm}$:
\begin{subequations}
\label{eq:change_per}
\begin{align}
& \phi_{x,i}^{-}=\gamma\mathcal{D}_{L}[\phi,\gamma](x_{i}) + \gamma\sum_{p=2}^{k}\sigma_{i,L}^{p-2}\mathcal{D}_{L}^{p}[\phi,\gamma](x_{i}),\\
& \phi_{x,i}^{+}=-\gamma\mathcal{D}_{R}[\phi,\gamma](x_{i}) - \gamma\sum_{p=2}^{k}\sigma_{i,R}^{p-2}\mathcal{D}_{R}^{p}[\phi,\gamma](x_{i});
\end{align}
\end{subequations}
while for non-periodic boundary conditions, \eqref{eq:partialsum_dir} are changed into
\begin{subequations}
	\label{eq:change_dir}
	\begin{align}
	& \phi_{x,i}^{-}=\gamma\mathcal{D}_{L}[\phi_{1,1},\gamma](x_{i}) + \gamma\sum_{p=2}^{k}\sigma_{i,L}^{p-2}\mathcal{D}_{L}[\phi_{1,p},\gamma](x_{i}),\\
	& \phi_{x,i}^{+}=-\gamma\mathcal{D}_{R}[\phi_{2,1},\gamma](x_{i}) - \gamma\sum_{p=2}^{k}\sigma_{i,R}^{p-2}\mathcal{D}_{R}[\phi_{2,1},\gamma](x_{i}).
	\end{align}
\end{subequations} 
Note that the WENO quadrature is only applied for approximating the operators with $p = 1$ in \eqref{eq:change_per}, and cheaper high order linear formula are used for those with $p>1$. The filter $\sigma_{i,L}$ and $\sigma_{i,R}$ are generated based on the smoothness indicators from the WENO methodology. 
%For brevity, we skip the details about the construction of the WENO quadrature as well as the nonlinear filter. All the formula have been well documented in \cite{christlieb2017kernel}.


Here, the fifth order WENO-based quadrature for approximating $J^{L}_{i}$ is provided as an example. The corresponding stencil is presented in Figure \ref{Fig0}. We choose the big stencil as $S(i)=\{x_{i-3},\ldots, x_{i+2}\}$ and the three small stencils as $S_{r}(i) =\{ x_{i-3+r},\ldots, x_{i+r}\}$, $r = 0, 1, 2$. For simplicity, we only provide the formulas for the case of a uniform mesh, i.e., $\Delta x_{i}=\Delta x$ for all $i$. Note that the WENO methodology is still applicable to the case of a nonuniform mesh, see \cite{shu2009high}. 

\begin{figure}
	\centering
	\includegraphics[width=0.5\textwidth]{figure/net.pdf}
	\caption{\em The structure of the stencils in WENO integration.   }
	\label{Fig0}
\end{figure}


\begin{enumerate}
	\item
	On each small stencil $S_{r}(i)$, we obtain the approximation as
	\begin{equation}
	\label{eq:weno1}
	J^{L}_{i,r} =\gamma \int_{x_{i-1}}^{x_{i}}e^{-\gamma(x_{i}-y)}p_{r}(y)dx,
	%=\sum_{j=0}^{k}c^{(r)}_{i-r-1+j}v_{i-r-1+j},
	\end{equation}
	where $p_{r}(x)$ is the polynomial interpolating $v(x)$ on nodes $S_{r}(i)$.
	
	\item
	Similarly, on the big stencil $S(i)$, we have
	\begin{equation}
	\label{eq:weno2}
	J^{L}_{i} =\gamma \int_{x_{i-1}}^{x_{i}}e^{-\gamma (x_{i}-y)}p(y)dx=\sum_{r=0}^{2}d_{r}J^{L}_{i,r},
	%=\sum_{j=0}^{2k-1}c_{i-k+j}v_{i-k+j},
	\end{equation}
	with the linear weights $d_{r}$ satisfying $\sum_{r=0}^{2}d_{r}=1$.
	
	\item
	We change the linear weights $d_{r}$ into the following nonlinear weights $\omega_{r}$, which are defined as
	\begin{equation}
	\omega_{r}=\tilde{\omega}_{r}/\sum\limits_{s=0}^{2}\tilde{\omega}_{s}, \ \ r=0,\ 1,\ 2,
	\end{equation}
	with
	\begin{equation*}
	\tilde{\omega}_{r}=d_{r}\left( 1+\frac{\tau_{5}}{\epsilon+\beta_{r}}\right) .
	\end{equation*}
	Here, $\epsilon>0$ is a small number to avoid the denominator becoming zero. We  take $\epsilon=10^{-6}$ in our numerical tests. The smoothness indicator $\beta_{r}$ is defined by
	\begin{equation}
	\beta_{r}=\sum_{l=2}^{3} \int_{x_{i-1}}^{x_{i}}\Delta x_{i}^{2l-3} \left(\frac{\partial^{l}p_{r}(x)}{\partial x^{l}}\right)^2 dx,
	\end{equation}
	which is used to  measure the relative smoothness of the function $v(x)$ in the stencil $S_{r}(i)$. In particular, we have the expressions as 
	\begin{subequations}
		\begin{align*}
		& \beta_{0} = \frac{13}{12} ( -v_{i-3} + 3v_{i-2} - 3v_{i-1} + v_{i} )^2
		+ \frac{1}{4} ( v_{i-3} - 5v_{i-2} + 7v_{i-1} - 3v_{i} )^2,\\
		& \beta_{1} = \frac{13}{12} (-v_{i-2} + 3v_{i-1} - 3v_{i} + v_{i+1} )^2
		+ \frac{1}{4} ( v_{i-2} - v_{i-1} - v_{i} + v_{i+1} )^2,\\
		& \beta_{2} = \frac{13}{12} (-v_{i-1} + 3v_{i} - 3v_{i+1} + v_{i+2} )^2 
		+ \frac{1}{4} (-3v_{i-1} + 7v_{i} - 5v_{i+1} + v_{i+2} )^2.
		\end{align*}
	\end{subequations}
	$\tau_{5}$ is simply defined as the absolute difference between $\beta_{0}$ and $\beta_{2}$ 
	$$\tau_{5}=|\beta_{0}-\beta_{2}|.$$
	Moreover, we define a parameter $\xi_{i}$ as
	\begin{align}
	\xi_{i}=\frac{\beta_{min}}{\beta_{max}},
	\end{align}
	which will be use to construct the nonlinear filter. Here,
	\begin{subequations}
		\begin{align*}
		\beta_{max} = 1 + \left(\frac{\tau_{5} }{  \epsilon + \min(\beta_{0},\beta_{2}) } \right)^2, \quad
		\beta_{min} = 1 + \left(\frac{\tau_{5} }{  \epsilon + \max(\beta_{0},\beta_{2}) } \right)^2.
		\end{align*}
	\end{subequations}
	Note that we have employed the nonlinear weights based on the idea of the WENO-Z scheme proposed in \cite{borges2008improved}, which enjoys less dissipation and higher resolution compared with the original WENO scheme.
	\item
	Lastly, we define the approximation
	\begin{equation}
	J^{L}_{i}=\sum_{r=0}^{2}\omega_{r}J^{L}_{i,r}.
	\end{equation}
	The filter $\sigma_{i,L}$ is defined as 
	\begin{align}
	\sigma_{i,L}=\min (\xi_{i-1}, \xi_{i}).
	\end{align}
	
\end{enumerate}


The process to obtain $J^{R}_{i}$ and $\sigma_{i,R}$ is mirror symmetric to that of $J^{L}_{i}$ and $\sigma_{i,L}$ with
respect to point $x_{i}$.


